Algorithms for Heavy-Tailed Statistics: Regression, Covariance Estimation, and Beyond

We study efficient algorithms for linear regression and covariance estimation in the absence of Gaussian assumptions on the underlying distributions of samples, making assumptions instead about only finitely-many moments. We focus on how many samples are needed to do estimation and regression with high accuracy and exponentially-good success probability. For covariance estimation, linear regression, and several other problems, estimators have recently been constructed with sample complexities and rates of error matching what is possible when the underlying distribution is Gaussian, but algorithms for these estimators require exponential time. We narrow the gap between the Gaussian and heavy-tailed settings for polynomial-time estimators with: 1. A polynomial-time estimator which takes $n$ samples from a random vector $X \in R^d$ with covariance $\Sigma$ and produces $\hat{\Sigma}$ such that in spectral norm $\|\hat{\Sigma} - \Sigma \|_2 \leq \tilde{O}(d^{3/4}/\sqrt{n})$ w.p. $1-2^{-d}$. The information-theoretically optimal error bound is $\tilde{O}(\sqrt{d/n})$; previous approaches to polynomial-time algorithms were stuck at $\tilde{O}(d/\sqrt{n})$. 2. A polynomial-time algorithm which takes $n$ samples $(X_i,Y_i)$ where $Y_i = \langle u,X_i \rangle + \varepsilon_i$ and produces $\hat{u}$ such that the loss $\|u - \hat{u}\|^2 \leq O(d/n)$ w.p. $1-2^{-d}$ for any $n \geq d^{3/2} \log(d)^{O(1)}$. This (information-theoretically optimal) error is achieved by inefficient algorithms for any $n \gg d$; previous polynomial-time algorithms suffer loss $\Omega(d^2/n)$ and require $n \gg d^2$. Our algorithms use degree-$8$ sum-of-squares semidefinite programs. We offer preliminary evidence that improving these rates of error in polynomial time is not possible in the median of means framework our algorithms employ.

==> content/certification.tex <==
\section{Certifying the Population Covariance}

\paragraph{Setup}
Let $v_1,\ldots,v_n$ be i.i.d. samples from a random vector $v$ on $\R^d$. We will make the following assumptions about $v$.
\begin{enumerate}
    \item $\E vv^\top = \Sigma$ (covariance exists)
    \item As a polynomial in $u = u_1,\ldots,u_d$, it holds that $\E_v \iprod{v,u}^4 \preceq O(1) \cdot (\E_v \iprod{v,u}^2)^2$. (Certifiable $4$-th moments; common assumption in SoS literature.)
    \item some $8$th moment assumption
\end{enumerate}

Let $\alpha > 0$ be a truncation level we will pick below.
Let $\tilde{v}_i = v_i \cdot \Ind[\|v_i\| \leq \alpha]$ be a truncated version of $v_i$.
Let $\tilde{\Sigma} = \E \tilde{v} \tilde{v}^\top$.
We will choose $\alpha$ such that $\|\tilde{\Sigma} - \Sigma\| \leq \text{small}$.
Fix $k \in N$ (later we will take $k = \Theta(\log(1/\delta))$).
Let $B_1,\ldots,B_k \subseteq [n]$ partition $n$ evenly into $k$ buckets.
For $i \leq k$, let
\[
Z_i = \frac k n \sum_{j \in B_i} \tilde{v_j}\tilde{v_j}^\top - \tilde{\Sigma} \mper
\]
We sometimes write $m = n/k$.

We want to find an SoS upper bound of $0.1k$ on the following polynomial system for the smallest $r$ we can.
Then this $r$ will be our error rate (up to constants).
\begin{align*}
  & \max_{b,u} \frac 1k \sum_{i=1}^k b_i \text{ such that}\\
  & b_i^2 = b_i \\
  & \|u\|^2 = 1 \\
  & b_i \iprod{Z_i, uu^\top} \geq r b_i\mper
\end{align*}
Like usual, we will use bounded differences to analyze concentration, so it will be enough to bound
\[
\E_v \max_{\pE} \frac 1k \pE \sum_{i=1}^k b_i \text{ s.t. $\pE$ satisfies above equations}
\]

\begin{lemma}\label[lemma]{lem:cert-main}
  If $r \geq ??$ then
  \[
  \E_v \max_{\pE} \frac 1k \pE \sum_{i=1}^k b_i \text{ s.t. $\pE$ satisfies above equations, degree $\pE = 4$}
  \]
  is at most $0.1k$.
\end{lemma}
To prove \cref{lem:cert-main} we need to assemble some other lemmas.

\begin{lemma}\label[lemma]{lem:expectation}
  Under our assumptions, for all degree-$4$ pseudodistributions,
  \[
  \pE_u \E_Z \iprod{Z \tensor Z, u^{\tensor 4}} \leq O(k/n) \|\Sigma\|^2
  \]
\end{lemma}
\begin{proof}
  Recall that $Z = \frac kn \sum_{i=1}^{n/k} \tilde{v_i}\tilde{v_i}^\top - \tilde{\Sigma}$ where $v_1,\ldots,v_{n/k}$ are i.i.d. samples from $v$.
  So
  \[
  \E Z \tensor Z = \frac {k^2}{n^2} \sum_{i=1}^{n/k} (\tilde{v_i}\tilde{v_i})^\top \tensor (\tilde{v_i}\tilde{v_i})^\top
  \]
  because the remaining terms are zero in expectation.
  By PSDness,
  \[
  \E \tilde{v_i}\tilde{v_i}^\top \tensor \tilde{v_i} \tilde{v_i}^\top \preceq \E v_i v_i^\top \tensor v_i v_i^\top
  \]
  and hence
  \[
  \E \iprod{Z \tensor Z, u^{\tensor 4}} \preceq \frac k n \E \iprod{v,u}^4 \preceq O(1) \cdot \frac k n \cdot (\E \iprod{v,u}^2)^2
  \]
\end{proof}

\begin{lemma}
  Let $Z = \frac 1m \sum_{i \leq m} \tilde{v_i}\tilde{v_i}^\top - \tilde{\Sigma}$.
  Then $\| \E ZZ^\top \tensor ZZ^\top \| \leq \|\Sigma\|^4 \Paren{\frac{d^3}{m^3} + \frac{d^2}{m^2}}$.
\end{lemma}
\begin{proof}
  If we expand $ZZ^\top \tensor ZZ^\top$, most terms zero in expectation.
  \[
  \E ZZ^\top \tensor ZZ^\top = \frac 1 {m^4} \Paren{m \E \|\tilde{v}\|^4 (\tilde{v}\tilde{v}^\top)^{\tensor 2} + m^2 \E \|\tilde{v_i}\|^2  v_i v_i^\top \tensor \|\tilde{v_j}\|^2 v_j v_j^\top + m^2 \E \iprod{v,w}^2 (v \tensor v)(w \tensor w)}
  \]
  NOTE: I LEFT SOME TERMS OUT HERE COMING FROM CENTERING; I THINK THEY ARE LOWER ORDER.
  Then by a Cauchy-Schwarz argument using $\E \iprod{v,u}^8 \leq \E (\iprod{v,u}^2)^4$, we get
  \[
  \| \E \|v\|^4 (vv^\top) \tensor (vv^\top) \| \leq \|\Sigma\|^4 \cdot d^3
  \]
  and similarly
  \[
  \| \E \|v\|^2 \|w\|^2 (vv^\top) \tensor (ww^\top) \| \leq \|\Sigma\|^4 \cdot d^2 
  \]
  NOTE: I THINK WE PROBABLY WANTED $\Tr \Sigma$ TO SHOW UP RATHER THAN $\|\Sigma\| d$ HERE -- MAYBE WE JUST NEED TO ADD AN ASSUMPTION THAT $\| \E \|v\|^2 (vv^\top \tensor vv^\top) \| \leq \Tr \Sigma \| \E (vv^\top \tensor vv^\top) \|$? OR MAYBE TRUNCATION WILL SAVE US?
  I think the remaining term is similar.
  So all in all, we get
  \[
  \| \E ZZ^\top \tensor ZZ^\top \| \leq \|\Sigma\|^4 \Paren{\frac{d^3}{m^3} + \frac{d^2}{m^2}}
  \]
\end{proof}

\begin{lemma}
  Let $\tau > 0$ and $\tilde{Z_i} = Z_i \cdot \Ind[\|Z_i\| \leq \tau]$.
  Then
  \[
  \E \Norm{ \sum_{i \leq k} \tilde{Z_i} \tensor \tilde{Z_i} - \E \tilde{Z_i} \tensor \tilde{Z_i} } \leq  O(\log(d)\tau^2) + O(\sqrt{k \log d}) \cdot \|\Sigma\|^2 \cdot \Paren{\frac{d^3}{m^3} + \frac{d^2}{m^2}}^{1/2}\mper
  \]
\end{lemma}
\begin{proof}
  We use matrix Bernstein.
  
  
  We have:
  \begin{align*}
    & \E \Norm{ \sum_{i \leq k} \tilde{Z_i} \tensor \tilde{Z_i} - \E \tilde{Z_i} \tensor \tilde{Z_i} }\\
    & \leq O(\log(d)) \tau^2 + O(\sqrt{\log(d)} \| \E \sum \tilde{Z_i}\tilde{Z_i}^\top \tensor \tilde{Z_i}\tilde{Z_i}^\top \|^{1/2}) \\
    & \leq O(\log(d)) \tau^2 + O(\sqrt{\log(d)} \| \E \sum Z_i Z_i^\top \tensor Z_i Z_i^\top \|^{1/2}) \\
    & \leq O(\log(d)) \tau^2 + O(\sqrt{k \log d}) \| \E Z Z^\top \tensor ZZ^\top \|^{1/2}
  \end{align*}
  where the second step is by PSDness and the third is because the $Z_i$'s are identically distributed.
  Now using the previous lemma to bound $\| \E ZZ^\top \tensor ZZ^\top \|$, we get a bound of
  \[
  O(\log(d)\tau^2) + O(\sqrt{k \log d}) \cdot \|\Sigma\|^4 \cdot \Paren{\frac{d^3}{m^3} + \frac{d^2}{m^2}}\mper
  \]
\end{proof}


\begin{proof}[Proof sketch of Lemma 1.1]
  Let's suppose that $\E \|Z\| \leq (\sqrt{d \|\Sigma\|} /m) \max(\sqrt{\Tr \Sigma}, \sqrt{m \|\Sigma\|})$. %Fill in details later for general truncated matrix variance + L4-L2 using matrix bernstein. 
  
  
  We can throw out the $Z_i$'s which are $100$ times larger, losing only $0.1k$ of them.
  Then we can set $\tau$ to the quantity above.
  For this sketch let's just suppose all the $Z_i$'s are this small.
  By standard Cauchy-Schwarz arguments, we can say
  \[
  \frac 1 k \pE \sum_{i=1} b_i \iprod{Z_i, uu^\top} \leq \frac 1 {\sqrt k} \Paren{\pE \sum \iprod{Z_i \tensor Z_i, u^{\tensor 4}}}^{1/2}\mper
  \]
  Now we can center $Z_i \tensor Z_i$.
  Using our SoS upper bound on $\E Z_i \tensor Z_i$, we get that the above is at most
  \[
  \frac 1 {\sqrt k} \Paren{ k^2 \|\Sigma\|^2 / n + \E \| \sum Z_i \tensor Z_i - \E Z_i \tensor Z_i \| }^{1/2}
  \]
  And then using our spectral bound, we get
  \[
  \frac 1 {\sqrt k} \Paren{ k^2 \|\Sigma\|^2 / n + O(\log (d) \tau^2) + O(\sqrt {k \log d}) \|\Sigma\|^2 (d^3/m^3 + d^2/m^2)^{1/2}}^{1/2}
  \]
\end{proof}



==> content/sosbernstein.tex <==
\section{SoS Matrix Bernstein}
\label[section]{sec:sosbernstein}

The key idea in the proof is to apply the standard Matrix Bernstein inequality to an appropriately preconditioned version of the matrix $M$. Effectively, this allows a sharper bound on the matrix variance-like term which can take advantage of the SoS certifiably-hypercontractive assumption as opposed to a cruder spectral norm bound.
\begin{lemma}[SoS Matrix Bernstein]
    \label{lem:sosmatbern}
  Let $M_i \in \R^{d^r \times d^r}$ be a sequence of i.i.d., mean-zero, random symmetric matrices satisfying the conditions,
  \begin{itemize}
      \item $\norm{M_i} \leq R$ almost surely,
      \item $\E[\langle u^{\otimes r}, M_i^2 u^{\otimes r} \rangle] \preceq \sigma^2 \norm{u}^{2r}$ where the left and right-hand sides are polynomials in $u$.
  \end{itemize}
  Then, 
  \begin{align}
      \E[ \max_{\tE} \tE[\sum_{i \leq k} \langle u^{\otimes r}, M_i u^{\otimes r} \rangle ] \leq \left( \frac{2 (\log(2) + r \log d)}{3} R + 2\sqrt{2k (\log(2) + r \log d)} \sigma \right) 
  \end{align}
  where the maxima is taken over all degree-$2r$ pseudoexpectations satisfying the polynomial inequality $\tE[\norm{u}^2]=1$.
\end{lemma}
\begin{proof}
We apply the standard matrix Bernstein inequality to the sum of random matrices $\sum_{i \leq k} M_i$ which has been preconditioned with the p.s.d. operator $A = \frac{1}{\sigma} \E[M^2] + \sigma \cdot I$, 
\begin{align*}
    \E[\norm{A^{-1/2} \sum_{i \leq k} M_i A^{-1/2}}] \leq \frac{1}{3} \log(2d^r) \max_i \norm{A^{-1/2} M_i A^{-1/2}} + \sqrt{2k \log(2d^r) \norm{\E[A^{-1/2} M A^{-1} M A^{-1/2}]}}.
\end{align*}
The fact that $A \succeq \sigma \cdot I \implies A^{-1} \preceq \frac{1}{\sigma} \cdot I \implies \norm{A^{-1/2}} \leq \frac{1}{\sqrt{\sigma}}$ and submultiplicativity of the operator norm show,
\begin{align*}
    \max_i \norm{A^{-1/2} M_i A^{-1/2}} \leq \max_i \norm{M_i} \norm{A^{-1/2}}^2 \leq  \frac{R}{\sigma}.
\end{align*}
We now bound the matrix variance term using the variational characterization of the operator norm and the Cauchy-Schwarz inequality,
\begin{align*}
    & \norm{\E[A^{-1/2} M A^{-1} M A^{-1/2}]} = \sup_{x : \norm{x}_2=1} \E[x^\top A^{-1/2} M A^{-1} M A^{-1/2} x] \leq \sup_{x : \norm{x}_2=1} \E[ \norm{x^\top A^{-1/2} M}   \norm{A^{-1}  M A^{-1/2}x}]  \\ & \leq \norm{A^{-1}} \sup_{x : \norm{x}_2=1} \E[ \norm{MA^{-1/2 }x}^2 ] \leq \norm{A^{-1}} \sup_{x : \norm{x}=1} x^\top A^{-1/2} \E[M^2] A^{-1/2} x] \leq \frac{1}{\sigma} \norm{A^{-1/2} \E[M^2] A^{-1/2}}.
\end{align*}
However note by construction that $\E[M^2] \preceq \sigma A \implies A^{-1/2} \E[M^2] A^{-1/2} \preceq \sigma I$, so $\norm{A^{-1/2} \E[M^2] A^{-1/2}} \leq \sigma$. Thus $\norm{\E[A^{-1/2} M A^{-1} M A^{-1/2}]} \leq 1$. Assembling, we conclude,
\begin{align*}
    \E \left[\norm{A^{-1/2} \sum_{i \leq k} M_i A^{-1/2}} \right] \leq \frac{\log(2d^r)}{3} \frac{R}{\sigma} + \sqrt{2k \log(2d^r)}
\end{align*}

To conclude our final result, note that the following inequality holds deterministically in the p.s.d. order,
\begin{align*}
    A^{-1/2} \sum_{i \leq k} M_i A^{-1/2} \preceq \norm{A^{-1/2} \sum_{i \leq k} M_i A^{-1/2}} \cdot I \implies \sum_{i \leq k} M_i \preceq A \norm{A^{-1/2} \sum_{i \leq k} M_i A^{-1/2}} 
\end{align*}
Noting $A \preceq B \implies \langle A, u^{\otimes k} \rangle \preceq \langle B, u^{\otimes k} \rangle$ (where the first $\preceq$ is in the semi-definite ordering and the second $\preceq$ corresponds to an SoS proof) applying the pseudoexpectation and expectation operators gives,
\begin{align*}
    & \max_{\tE} \tE \langle u^{\otimes r}, \sum_{i \leq k} M_i u^{\otimes r} \rangle \leq \norm{A^{-1/2} \sum_{i \leq k} M_i A^{-1/2}} \cdot \max_{\tE} \tE \langle u^{\otimes r}, \sum_{i \leq k} A u^{\otimes r} \rangle \implies \\
    & \E[\max_{\tE} \tE \langle u^{\otimes r}, \sum_{i \leq k} M_i u^{\otimes r} \rangle] \leq \E[\norm{A^{-1/2} \sum_{i \leq k} M_i A^{-1/2}}] \cdot \max_{\tE} \tE \langle u^{\otimes r}, \sum_{i \leq k} A u^{\otimes r} \rangle \\
    & \leq \left(\frac{2 (\log(2) + r \log d))}{3} R + 2\sqrt{2k (\log(2) + r \log d)} \sigma \right) \max_{\tE} \tE[\norm{u}^{2k}]
\end{align*}
using the result of the previous matrix Bernstein bound and the SoS hypercontractivity assumption. Finally note $\max_{\tE} \tE[\norm{u}^{2k}]=1$ under the conditions of the theorem.
\end{proof}

% \Nnote{Comments. Change Def 3.2 to certifiable, L8-L2 hypercontraction so correct definition is cited. Also state and prove lemma for truncated Z. That is let $\tZ_i = \frac{1}{m} (\tv_i \tv_i - \Sigma) \Ind[\norm{Z_i} \geq \tau]$ (just need to briefly argue removing the truncations only makes terms bigger). Also in final statement would just directly compute $\E [\norm{v}^8])^{1 / 2} (\pE \E [\iprod{u, v}^8])^{1 / 2} $ explicitly. The 8th moment bound is in the appendix somewhere so you can just cite it. Basically just want lemma to match Lemma 4.5}. 
\begin{lemma}
    \label{lem:sosmvbound}
    Consider the random matrix, $Z = \frac{1}{m} \sum_{i = 1}^m (\tv_i \tv_i^\top - \tilde{\Sigma})$ where $\tv_i = v_i \Ind[\norm{v_i} \leq \alpha]$ and $v_i$ are drawn i.i.d. from a distribution $\mathcal{D}$ satisfying \cref{def:nice-dist} with covariance matrix $\Sigma$. Let $\tZ = Z \Ind[\norm{Z} \leq \tau]$.  Then, we have that for any pseudoexpectation, $\pE$, satisfying $\norm{u}^2 = 1$:
    \begin{equation*}
        \pE \iprod{\E [\tZ^2 \tensor \tZ^2] - (\E [\tZ \tensor \tZ])^2, u^{\tensor 4}} \leq O \Paren{\frac{1}{m^2}} L^2 (\Tr \Sigma)^2 \norm{\Sigma}^2.
    \end{equation*}
\end{lemma}

\begin{proof}
Firstly, we have:
\begin{equation*}
    \pE \iprod{(\E [\tZ \tensor \tZ])^2, u^{\tensor 4}} = \pE \iprod{(u^{\tensor 2})^\top(\E [\tZ \tensor \tZ])^2, u^{\tensor 2}} \geq 0.
\end{equation*}
Therefore, we can ignore the second term in the inner product. From this, we get from the fact that $Z^2 \tensor Z^2$ is positive semidefinite:
\begin{equation*}
    \pE \iprod{\E [\tZ^2 \tensor \tZ^2] - (\E [\tZ \tensor \tZ])^2, u^{\tensor 4}} \leq \pE \iprod{\E [\tZ^2 \tensor \tZ^2], u^{\tensor 4}} = \pE \iprod{\E [Z^2 \tensor Z^2 \Ind[\norm{Z} \leq \tau]], u^{\tensor 4}} \leq \pE \iprod{\E [Z^2 \tensor Z^2], u^{\tensor 4}}.
\end{equation*}
We now expand the right hand side as follows:
\begin{align*}
    \pE \iprod{\E [Z^2 \tensor Z^2], u^{\tensor 4}} &= \frac{1}{m^3} \pE \Iprod{\E [((\tv\tv^\top - \tSigma)^2)^{\tensor 2}], u^{\tensor 4}} + O \Paren{\frac{1}{m^2}} \pE \Iprod{\E [((\tv\tv^\top - \tSigma)^2) \tensor ((\tw\tw^\top - \tSigma)^2)], u^{\tensor 4}}\\
    &+ O \Paren{\frac{1}{m^2}} \pE \Iprod{\E [((\tv\tv^\top - \tSigma) (\tw\tw^\top - \tSigma)) \tensor ((\tw\tw^\top - \tSigma) (\tv\tv^\top - \tSigma)))], u^{\tensor 4}} \\
    &+ O \Paren{\frac{1}{m^2}} \pE \Iprod{\E [((\tv\tv^\top - \tSigma) (\tw\tw^\top - \tSigma))^{\tensor 2})], u^{\tensor 4}}.
\end{align*}
Note, that all other terms that arise vanish under expectations. For the first term, we have:
\begin{align*}
    \pE \Iprod{\E [((\tv\tv^\top - \tSigma)^2)^{\tensor 2}], u^{\tensor 4}} &= \pE \E [(u^\top (\tv\tv^\top - \tSigma)^2 u)^2] = \pE \E [(\norm{\tv}^2 \iprod{u, \tv}^2 -2 \iprod{\tv, u} \tv^\top \tSigma \tv + u^\top \tSigma^2 u)^2] \\
    &\leq \pE \E [(2\norm{\tv}^2 \iprod{u, \tv}^2 + 2 u^\top \tSigma^2 u)^2] \leq 4 \pE \E [2(\norm{\tv}^2 \iprod{u, \tv}^2)^2 + 2 (u^\top \tSigma^2 u)^2] \\
    &\leq 8 \pE \E [\norm{\tv}^4 \iprod{u, \tv}^4 + (u^\top \tSigma^2 u)^2] \leq 8 \pE \E [\norm{\tv}^4 \iprod{u, \tv}^4] + 8\norm{\tSigma}^4 \\
    &\leq 8 (\E [\norm{\tv}^8])^{1 / 2} (\pE \E [\iprod{u, \tv}^8])^{1 / 2} + 8\norm{\tSigma}^4.
\end{align*}
For the second term, we have:
\begin{align*}
    &\pE \Iprod{\E [((\tv\tv^\top - \tSigma)^2) \tensor ((\tw\tw^\top - \tSigma)^2)], u^{\tensor 4}} = \pE \E [(u^\top(\tv\tv^\top - \tSigma)^2u) (u^\top(\tw\tw^\top - \tSigma)^2 u)] \\
    &\qquad \leq \frac{1}{2} \cdot \pE \E [(u^\top(\tv\tv^\top - \tSigma)^2u)^2 + (u^\top(\tw\tw^\top - \tSigma)^2 u)^2] = \pE \E [(u^\top(\tv\tv^\top - \tSigma)^2u)^2] \\
    &\qquad \leq 8 (\E [\norm{\tv}^8])^{1 / 2} (\pE \E [\iprod{u, \tv}^8])^{1 / 2} + 8\norm{\tSigma}^4.
\end{align*}
Similarly, for the third term, we get:
\begin{align*}
    &\pE \Iprod{\E [((\tv\tv^\top - \tSigma) (\tw\tw^\top - \tSigma)) \tensor ((\tw\tw^\top - \tSigma) (\tv\tv^\top - \tSigma)))], u^{\tensor 4}} \\
    &\qquad = \pE \E [(u^\top (\tv\tv^\top - \tSigma) (\tw\tw^\top - \tSigma)u) (u^\top (\tw\tw^\top - \tSigma) (\tv\tv^\top - \tSigma)u))] \\
    &\qquad = \pE \E [(u^\top (\tv\tv^\top - \tSigma) (\tw\tw^\top - \tSigma)u)^2] \leq \pE \E [(u^\top (\tv\tv^\top - \tSigma)^2u) \cdot (u^\top (\tw\tw^\top - \tSigma)^2 u)] \\
    &\qquad \leq \frac{1}{2} \cdot \pE \E [(u^\top (\tv\tv^\top - \tSigma)^2u)^2 + (u^\top (\tw\tw^\top - \tSigma)^2u)^2] \leq 8 (\E [\norm{\tv}^8])^{1 / 2} (\pE \E [\iprod{u, \tv}^8])^{1 / 2} + 8\norm{\tSigma}^4.
\end{align*}
Finally, for the last term, we notice that:
\begin{equation*}
    \pE \Iprod{\E [((\tv\tv^\top - \tSigma) (\tw\tw^\top - \tSigma))^{\tensor 2})], u^{\tensor 4}} = \pE \E [(u^\top (\tv\tv^\top - \tSigma) (\tw\tw^\top - \tSigma)u)^2].
\end{equation*}
Finally, we have:
\begin{equation*}
    \E [\norm{\tv}^8] = \E [\norm{v}^8 \Ind[\norm{v} \leq \alpha]] \leq \E [\norm{v}^8] \text{ and } \norm{\tSigma} = \max_{\norm{u} = 1} \E [\iprod{u, v}^2 \Ind[\norm{v} \leq \alpha]] \leq \max_{\norm{u} = 1} \E [\iprod{u, v}^2] = \norm{\Sigma}.
\end{equation*}
Similarly, we also have from the fact that $\iprod{v, u}^8$ is a square polynomial:
\begin{equation*}
    \pE \E [\iprod{u, \tv}^8] = \pE \E [\iprod{u, v}^8 \Ind[\norm{v} \leq \alpha]] \leq \pE \E [\iprod{u, v}^8].
\end{equation*}
From \cref{lem:l8l2vec} and the certifiable hypercontractivity of $\mathcal{D}$, this concludes the proof of the lemma.
\end{proof}

\begin{lemma}
  \label[lemma]{lem:p-main-sharp}
  Let $v_1,\ldots,v_n \sim \cD$ be i.i.d and assume the distribution $\cD$ satisfies \cref{def:nice-dist}.
  Then for $p$ as in \eqref{eq:p-def},
  \begin{align*}
  & \E_{v_1,\ldots,v_n} \Brac{ \max_{\pE_u} \pE_u p(u) } \\
  & \leq O\Paren{\frac 1 n \cdot k^{3/2} \cdot L \cdot \Tr \Sigma \cdot \Brac{\|\Sigma\|_2 + \sqrt{\frac k n} \cdot \|\Sigma\|_F} \cdot \sqrt{\log d} } + O \Paren{ \frac{k^2}{n} \cdot L \cdot \|\Sigma\|_2^2} + O \Paren{\tau^2 \cdot \log d}\mper
  \end{align*}
  where the maximum is over all degree-$4$ pseudodistributions in variables $u = (u_1,\ldots,u_d)$ satisfying $\{\|u\|^2 = 1\}$.
\end{lemma}

\begin{lemma}\label[lemma]{lem:cert-main-sharp} Assume that the $v_i$ are $L$-nice,
fix $k \in \mathbb{N}$ and
let $B_1,\ldots,B_k \subseteq [n]$ partition $n$ evenly into $k$ buckets. 
For $i \leq k$, let $Z_i = \frac k n \sum_{j \in B_i} \tv_j\tv_j^\top - \tilde{\Sigma}$ where $\tv_i = v_i \Ind[\normt{v_i} \leq \alpha]$.
If the truncation level $\alpha = \left( \frac{\normt{\Sigma} \cdot L^{3/2} }{\Tr(\Sigma)} \cdot \frac{n}{\sqrt{k}} \right)^{1/6} \cdot \sqrt{\Tr(\Sigma)}$ and
  if $r \geq \tilde{O} \left( \frac{L \normt{\Sigma}}{\sqrt{n}} \left( \frac{k^{1/3} \sr^{2/3}}{n^{1/6}} + \frac{\sr^{3/4} \sqrt{k}}{n^{1/4}} +  k^{1/4} \sr^{1/2} + \sqrt{k} \right) \right)$ then
  \[
  \max_{\pE} \frac 1k \pE \sum_{i=1}^k b_i \text{ s.t. $\pE$ satisfies \ref{eq:tstco}$( r, \bZ)$ and degree $\pE = 4$}
  \]
  is at most $0.001$ with probability at least $1-2^{-\Omega(k)}$.
\end{lemma}

\begin{proof}[Proof of \cref{lem:cert-main-sharp}]

The primary technical challenge is bounding the expected value of the (random) SoS program in \ref{eq:tstco} since concentration around this expected value follows by a bounded differences argument. Accordingly we begin by bounding the expected value $\E_v \max_{\pE} \frac 1k \pE \sum_{i=1}^k b_i$.

To begin, simply for the purposes of our analysis, we partition the set of $k$ indices corresponding to buckets $B_1, \hdots, B_k$, into two sets, $\cG = \{i : \normt{Z_i} \leq \tau\}$ and $\cB = \{i : \normt{Z_i} > \tau\}$. Then, for any degree-4 $\pE$ satisfying the constraints in \ref{eq:tstco}, we have that
\begin{align*}
\E_v \max_{\pE} \frac 1k \pE \sum_{i=1}^k b_i \leq \E_v \max_{\pE} \frac 1k \pE \sum_{i \in \cG} b_i + \E_v \max_{\pE} \frac 1k \pE \sum_{i \in \cB} b_i.
\end{align*}
Now, since $\E \normt{Z} \leq  O(\log d) \frac{\alpha^2}{m} + O(\sqrt{\log d/m}) \sqrt{L \Tr \Sigma \normt{\Sigma}}$ (which follows from \cref{lem:EZub}), taking $\tau = C_1 \left( \log(d) \frac{\alpha^2}{m} + \sqrt{\log (d)} \sqrt{L \Tr \Sigma \normt{\Sigma}/m} \right)$ for some large-enough constant $C_1$, we can ensure that
\begin{align*}
    \E_v \max_{\pE} \frac 1k \pE \sum_{i \in \cB} b_i \leq \E_v \frac{1}{k} \sum_{i \leq k} \Ind[\normt{Z_i} \geq \tau] \leq \frac{1}{k} \frac{\sum_{i \leq k} \E \normt{Z_i}}{\tau} \leq .00025
\end{align*}
since $\pE[b_i] \leq 1$ and by appealing to Markov's inequality. For the remainder of the argument we fix this truncation level $\tau$. Now to control $\E_v \max_{\pE} \frac 1k \pE \sum_{i \in \cG} b_i$ we have that, 
\begin{align*}
    \E_v \max_{\pE} \frac 1k \pE \sum_{i \in \cG} b_i \leq \frac{1}{r} \E_v \max_{\pE} \frac 1k \pE \sum_{i \in \cG} b_i \iprod{Z_i, uu^\top} = \frac{1}{r} \E_v \max_{\pE} \frac 1k \pE \sum_{i \in \cG} b_i \iprod{\tZ_i, uu^\top}
\end{align*}
using the constraints in \ref{eq:tstco} and defining $\tZ_i = Z_i \Ind[\normt{Z_i} \leq \tau]$. Now by an application of the SoS Cauchy-Schwarz inequality, we have
  \[
  \frac 1 k \E_v \max_{\pE} \pE \sum_{i \in \cG} b_i \iprod{\tZ_i, uu^\top} \leq \frac 1 {\sqrt k} \Paren{\E_v \max_{\pE} \pE \sum_{i=1}^k \iprod{\tZ_i \tensor \tZ_i, uu^\top \tensor uu^\top}}^{1/2}\mper
  \]
  Now using sub-additivity of the $\sqrt{\cdot}$,
  \begin{align*}
  & \frac 1 {\sqrt k}  \Paren{\E_v \max_{\pE} \pE \sum_{i=1}^k \iprod{\tZ_i \tensor \tZ_i, uu^\top \tensor uu^\top}}^{1/2} \leq \\
  & \frac{1}{\sqrt{k}}  \Paren{ O(\log(d)\tau^2) + O(\sqrt{k \log d}) \cdot \sqrt{O \left(\frac{1}{m^3} L^2 \Tr(\Sigma)^2 \norm{\Sigma}_F^2 + \frac{1}{m^2} L^2 \normt{\Sigma}^2 \Tr(\Sigma)^2 \right)} }^{1/2} + \\
  & \frac{1}{\sqrt{k}} \left(O(\frac{L k}{m}) \cdot \normt{\Sigma}^2 \right)^{1/2}.
  \end{align*}
  for any degree-4 $\pE$ satisfying the conditions of the theorem by \cref{lem:p-main}.
  Note that $\tau$ is a function of the truncation level $\alpha$ on the vectors $v_i$. We now choose $\alpha$ appropriate to balance the bias from truncation and the previous upper bound. For convenience we reparametrize as $\alpha = \beta \sqrt{\Tr \Sigma}$. Recall by \cref{lem:bias} we have that our bias is $\normt{\tSigma-\Sigma} \leq \frac{L^{3/2} \normt{\Sigma}}{\beta^4} \equiv B(\beta)$. Similarly, after algebraic simplifications we obtain that aforementioned upper bound is at most,
  \begin{align*}
      & \log(d)^{3/2} \cdot O \Big( \sqrt{k} \frac{\Tr(\Sigma) \beta^2}{n} + \frac{1}{\sqrt{n}} \sqrt{L \Tr(\Sigma) \normt{\Sigma}} +  \\
      &  \sqrt{k} \cdot \frac{\sqrt{L \Tr(\Sigma) \norm{\Sigma}_F}}{n^{3/4}} + k^{1/4} \frac{\sqrt{L \normt{\Sigma} \Tr(\Sigma)}}{\sqrt{n}} + \sqrt{\frac{kL}{n}} \normt{\Sigma} \Big).
  \end{align*}
  where we have used that $m=n/k$ and define $$R(\beta) = \sqrt{k} \frac{\Tr(\Sigma) \beta^2}{n} + \frac{1}{\sqrt{n}} \sqrt{L \Tr(\Sigma) \normt{\Sigma}} +  \sqrt{k} \cdot \frac{\sqrt{L \Tr(\Sigma) \norm{\Sigma}_F}}{n^{3/4}} + k^{1/4} \frac{\sqrt{L \normt{\Sigma} \Tr(\Sigma)}}{\sqrt{n}} + \sqrt{\frac{kL}{n}} \normt{\Sigma}$$ for convenience.
  Since our final estimation error for $\Sigma$ will be upper bounded by $O(\log(d)^{3/2} R(\beta)+B(\beta)) \leq C_2 \log(d)^{3/2} (R(\beta)+B(\beta))$ for some universal constant $C_2$, we choose $\beta$ minimize $R(\beta)+B(\beta)$. A short computation choosing $\beta$ to balance the first term in $R(\beta)$ and $B(\beta)$ shows the optimal $\beta^* = \left (\frac{\normt{\Sigma} \cdot L^{3/2} }{\Tr(\Sigma)} \cdot \frac{n}{\sqrt{k}} \right)^{1/6}$. Hence we have the final rate can be upper bounded, 
  \begin{align*}
    \tilde{O} \left( \frac{L \normt{\Sigma}}{\sqrt{n}} \left( \frac{k^{1/3} \sr^{2/3}}{n^{1/6}} + \frac{\sr^{3/4} \sqrt{k}}{n^{1/4}} +  k^{1/4} \sr^{1/2} + \sqrt{k} \right) \right)
  \end{align*}
  where we have used that $\norm{\Sigma}_F^2 \leq \Tr(\Sigma) \cdot \normt{\Sigma}$. By assembling this bound with our previous results and choosing $r \geq \tilde{O} \left( \frac{L \normt{\Sigma}}{\sqrt{n}} \left( \frac{k^{1/3} \sr^{2/3}}{n^{1/6}} + \frac{\sr^{3/4} \sqrt{k}}{n^{1/4}} +  k^{1/4} \sr^{1/2} + \sqrt{k} \right) \right)$, with appropriately large constant in the $\tilde{O}$, we can guarantee that 
  \begin{align*}
  \E_v \max_{\pE} \frac 1k \pE \sum_{i=1}^k b_i \leq .0005
  \end{align*}
  where $\max_{\pE}$ is taken over any degree-4 pseudoexpecation $\pE$ satisfying the constraints in \ref{eq:tstco}. 
  
  Finally, since by \cref{lem:sos-conc}, \ref{eq:tstco} obeys a bounded-difference condition, simply applying the bounded differences inequality shows that under the previous conditions,
  \begin{align*}
      \max_{\pE} \frac 1k \pE \sum_{i=1}^k b_i \leq .001
  \end{align*}
  with probability at least $1-2^{-\Omega(k)}$.
\end{proof}

